Perturbation of error bounds

Our aim in the current article is to extend the developments in Kruger, Ngai & Th\'era, SIAM J. Optim. 20(6), 3280-3296 (2010) and, more precisely, to characterize, in the Banach space setting, the stability of the local and global error bound property of inequalities determined by proper lower semicontinuous under data perturbations. We propose new concepts of (arbitrary, convex and linear) perturbations of the given function defining the system under consideration, which turn out to be a useful tool in our analysis. The characterizations of error bounds for families of perturbations can be interpreted as estimates of the `radius of error bounds'. The definitions and characterizations are illustrated by examples.

==> KLTIntro9.tex <==
\section{Introduction and Preliminaries}
In this article, we mostly follow the standard terminology and notation used by the optimization and variational analysis community, see,  e.g., \cite{RocWet98,DonRoc14}.
Throughout, $X$ and $X^*$ stand for a real Banach space and its topological dual, respectively, while $\B$ and $\B^*$ denote the corresponding unit balls.
The norms in both spaces are denoted by the same symbol $\Vert\cdot\Vert$.
For a subset $S$, we denote its interior and boundary by $\Int S$ and $\bd S$, respectively.
The distance from a point $x$ to a set $S$ is denoted by $d(x,S):=\inf_{u\in S}\Vert u-x\Vert$, and we use the con\-vention $d(x,S)=+\infty$  whenever   $S=\emptyset$.

For an extended-real-valued  function: $f : X\rightarrow\R_\infty:=\R\cup\{+\infty\}$, its domain is the set
$\dom f:=\{x\in X\mid f(x) < +\infty\}$.
A function $f$ is said to be \emph{proper} if
%it is not identically $-\infty$ and
$\dom f\ne\emptyset$.
We use the symbol $f_+(x)$ to denote $\max(f(x),0)$.
The class of all extended-real-va\-lued proper convex lower semicontinuous functions on $X$ is denoted by $\Gamma_0(X)$.
For a convex function $f:X\to {\R_\infty}$, its (Moreau) \emph{subdifferential} at $x\in\dom f$ is given by
$$\partial  f(x):=\{x^*\in X^*\mid  \langle x^{\star},u-x\rangle\le f(u)-f(x),\; \forall u\in X\}.$$
It is a (possibly empty) weak$^*$-closed set in $X^*$.

The article is  concerned with the study of the solution set of a single inequality of the type
\begin{equation}\label{2}
S_f:=\{x\in X\mid f(x)\le 0\},
\end{equation}
where $f:X\rightarrow\R_\infty$.
Such sets subsume, e.g., feasible sets in mathematical programming.
Indeed, solutions of a finite family of inequalities:
\begin{equation*}\label{l2bis}
\{x\in X\mid f_i(x)\leq 0\quad \text{ for all} \quad i=1,\ldots, n\}
\end{equation*}
can be re\-written as (\ref{2}) with function $f$ defined by
$f(x)=\max\{f_1(x),\ldots,f_n(x)\}$.

An important issue when studying  systems  of the type (\ref{2}) is to give an upper estimate (error bound) of the distance from a point $x\in X$  to the set $S_f$ in terms of a  computable function measuring the violation of the inequality in \eqref{2}.
This can, e.g., be the function $f$ itself.

We say that a function $f$ has (or admits) a {\it local error bound} at a point $\bar x \in S_f$ if there exists a real $\tau>0$ such that
\begin{equation}\label{4}
\tau d(x,S_f) \leq f_+(x)
\end{equation}
for all $x$ near $\bar x$.
We similarly say that a function $f$ has a \textit{global error bound} if there exists a real $\tau>0$ such that inequality (\ref{4}) is satisfied for all $x\in X$.

The exact upper
bound of all such $\tau$ (the \textit{error bound modulus}; cf. \cite{FabHenKruOut10}) equals either \begin{equation}\label{ErL}
\Er{f}(\bar{x}) :=\liminf_{\gfrac{x\to\bar{x}}{f(x)>0}}
\frac{f(x)}{d(x,S_f)}
\end{equation}
in the local setting, or
\begin{equation}\label{ErG}
\Er{f}:=\inf_{f(x)>0} \frac{f(x)}{d(x,S_f)}
\end{equation}
in the global case.
Constants (\ref{ErL}) and (\ref{ErG}) provide
quantitative estimates of the error bound property.

The starting point of the theory  of error bounds goes back to the pio\-neering work  by Hoffman \cite{Hof52} (although some traces of the error bound property can be found in an earlier publication by Rosenbloom \cite{Ros51}\footnote{Private communication by J.-B. Hiriart-Urruty})
who established for a linear function in finite di\-mensions the following result:
\vskip 2mm
\textit{ Given an $m\times n$  matrix $A$ and a vector $b\in \R^m$, there exists a positive number $\kappa > 0 $ such that the distance from $x$ to the set $S:=\{x\in\R^n\mid  Ax\leq b\} $  has an upper bound given  by $\kappa \Vert (Ax-b)_+\Vert$, where  for  $y:=(y_1,\ldots,y_m)\in \R^m$,  $y_+$ denotes the vector  $(\max(y_1,0),\ldots,\max(y_m,0))$.}
\vskip 2mm

%In other words, the distance from a point $x\in \R^n$  to the solution set of a system of linear inequalities (the error) is bounded above by a constant times the norm of the residual.
%By a residual we mean a function $r:\R^m\to\R_+$  such that $r(x) = 0$ if and only if $x$ belongs to the solution set.

After the work by Hoffmann and its extensions by Robinson \cite{Rob75}, Man\-gasarian \cite{Man85}, Auslender \& Crouzeix \cite{AusCro88}, Pang \cite{Pang97}, Lewis and Pang \cite{LewPan98}, Klatte \& Li \cite{KlaLi99}, Jourani \cite{Jou00}, there have been significant developments of various aspects of errors bounds for con\-vex and nonconvex functions in recent years.
The interested reader is referred to the articles by Ng \& Zheng \cite{NgZhe01}, Az{\'e} \cite{Aze03,Aze06}, Az{\'e} \& Corvellec \cite{AzeCor04}, Z{\u{a}}linescu \cite{Zal03}, Huang \& Ng \cite{HuaNg04}, Corvellec \& Motreanu \cite{CorMot08}, Fabian et al \cite{FabHenKruOut10,FabHenKruOut12}, Gfrerer \cite{Gfr11}, Ioffe \cite{Iof00_,Iof}, Ioffe \& Outrata \cite{IofOut08}, Ngai \& Th{\'e}ra \cite{NgaiThe04,NgaiThe05,NgaiThe08,NgaiThe09}, Zheng \& Ng \cite{ZheNg10,ZheNg12}, Bednarczuk \& Kruger \cite{BedKru12,BedKru12.2}, Meng \& Yang \cite{MenYan12}, Kruger \cite{Kru15,Kru15.2,Kru15.3} and the references therein.

Many authors have recently studied
error bounds   in connection with the \emph{metric regularity} and \emph{subregularity} (cf. \cite{DonRoc14}) as well as \emph{Aubin property} and \emph{calmness} of set-valued mappings: \cite{Aze06,CanKruLopParThe14,CanHenLopPar16,Gfr11,Iof00_,Iof, IofOut08, NgaiThe04,NgaiThe08,Kru15,Kru15.2,Kru15.3,ZheNg10,ZheNg12, NgaiTronThe13,NgaiTronThe14}.
The connections between the error bounds and weak sharp minima were studied in \cite{BurDeng05}.


Another typical example where the theory of error bounds plays an important role  is the so-called \textit{feasibility problem} \cite{BauBor96, BecTeb03, HesLuk13, KruLukTha}, which consists in finding a point in the intersection of a finite family  of  closed (usually convex) sets and has a broad applicability in various areas such as, e.g., image reconstruction \cite{Com96}.
Several iterative methods such as the method of successive orthogonal projections, the cyclic subgradient projections method, etc,  are known to solve this problem (see \cite{Cen84}).
Error bounds are also used in the convergence analysis of projection algorithms.
They allow one to quantify the proximity of an iterate to the solution set of the problem.
The reader is referred to the recent survey paper by Ioffe \cite{Iof,Iof2} and the references therein and also to some recent contributions  by Beck \& Teboulle \cite{BecTeb03}, Lewis et al \cite{LewLukMal09}, Hesse \& Luke \cite{HesLuk13}, Borwein et al \cite{BorLiYao14}, Drusvyatskiy et al \cite{DruIofLew15.2}, Kruger \& Thao \cite{KruTha16}, Noll \& Rondepierre \cite{NolRon16}, and Bolte et al \cite{BolNguPeySut}.

In this article, we
%mainly
study stability of local and global error bounds under perturbations.
%More precisely,
It was  observed in Ngai et al \cite[Theorem~1]{NgaiKruThe10} and Kruger et al \cite[Theorem~1]{KruNgaiThe10}, that the requirement for the distance from the origin to the subdifferential of a function at a reference point to be strictly positive, while being a conventional sufficient condition for a local error bound for the system (\ref{2}), is far from being necessary.
This con\-dition guaranties the local error bound property not just for the given function, but also for a family of its small per\-turbations.
In Section~\ref{On}, we exploit the concept of local $\varepsilon$-perturbation from \cite{KruNgaiThe10}, define subfamilies of convex and linear $\varepsilon$-perturbations, and establish in Theorem~\ref{ge} the exact formula for the `radius of  local error bounds'  for families of  arbitrary, convex and linear perturbations in terms of the distance from the origin to the subdifferential.

\red{
Theorem~\ref{ge} in a sense continues the series of \emph{radius theorems} from Dontchev--Rockafellar \cite{DonRoc14}, ``furnishing
a bound on how far perturbations of some sort in the specification of a problem can
go before some key property is lost'' \cite[page~364]{DonRoc14}.
Note that, unlike the `stable' properties of \emph{metric regularity}, \emph{strong metric regularity} and \emph{strong metric subregularity} studied in \cite{DonRoc14}, the error bound property (as well as the equivalent to it metric subregularity property, cf. \cite[page~200]{DonRoc14}) can be lost under infinitely small perturbations.
That is why stronger conditions are required to ensure stability.
Unlike, e.g., \cite[Theorem~6A.9]{DonRoc14} which gives the radius of strong metric subregularity in terms of the \emph{subregularity modulus} being an analogue of (the reciprocal of) the error bound modulus $\Er{f}(\bar{x})$ \eqref{ErL}, Theorem~\ref{ge} utilizes the quantity $\varsigma(f,\bar{x})$ (see Theorem~\ref{lo} below).
In view of Theorem~\ref{lo}, this quantity can be smaller than $\Er{f}(\bar{x})$, and, thus, condition $\varsigma(f,\bar{x})>0$ used in Corollary~\ref{re} imposes a strong requirement on the function $f$ and $\varsigma(f,\bar{x})$ leads to a radius theorem of a different type compared to those in \cite{DonRoc14}.
}

The same idea applies partially when considering stability of global error bounds in Section~\ref{S3}.
In the global setting, we define families of convex and linear perturbations as well as larger families of weak convex and weak linear perturbations, discuss some limitations of these definitions, and establish in Theorem~\ref{Ge} lower and upper estimates for the `radius of global error bounds'  for families of such perturbations.
The family of convex perturbations considered here is larger than the corresponding one studied in \cite{KruNgaiThe10}.
In particular, the so called \emph{asymptotic
qualification condition} is waived.

Some examples are given for the convenience of the reader to illustrate the different concepts introduced along the presentation.

